Flexible Instruction-Set Semantics via Type Classes

Instruction sets, from families like x86 and ARM, are at the center of many ambitious formal-methods projects. Many verification, synthesis, programming, and debugging tools rely on formal semantics of instruction sets, but different tools can use semantics in rather different ways. As a result, a central challenge for that community is how semantics should be written and what techniques should be used to connect them to new use cases. The best-known work applying single semantics across quite-different tools relies on domain-specific languages like Sail, where the language and its translation tools are specialized to the realm of instruction sets. We decided to explore a different approach, with semantics written in a carefully chosen subset of Haskell. This style does not depend on any new language translators, relying instead on parameterization of semantics over type-class instances. As a result, a semantics can be a first-class object within a logic, and application of a semantics for a new kind of tool can be a first-class operation in the logic, allowing sharing of theorems across applications. Our case study is for the open RISC-V instruction-set family, and we have used a single core semantics to support testing, interactive proof, and model checking of both software and hardware. We especially highlight an application of a first-class semantics within Coq that can be instantiated in different ways within one proof: simulation between variants where multiplication is implemented in hardware or in the machine code of a particular software trap handler.

==> data/loc.tex <==
\begin{tabular}{lr}
\toprule
Spec part       &  LOC \\
\midrule
Primitives      &  165 \\
Decode          &  625 \\
CSR fields      &  509 \\
Execute         &  939 \\
Utilities       &  224 \\
\midrule
Total           & 2462 \\
\bottomrule
\end{tabular}
\hspace{2em}
\begin{tabular}{lr}
\toprule
Use case        &  LOC \\
\midrule
Simulator       &  480 \\
riscv-tests     &  108 \\
Clash           &  235 \\
Gcd             &   25 \\
WMM             &  738 \\
\midrule
Total           & 1586 \\
\bottomrule
\end{tabular}

\todo{also count ???}

